Dual Task Framework for Improving Persona-grounded Dialogue Dataset

This paper introduces a simple yet effective data-centric approach for the task of improving persona-conditioned dialogue agents. Prior model-centric approaches unquestioningly depend on the raw crowdsourced benchmark datasets such as Persona-Chat. In contrast, we aim to fix annotation artifacts in benchmarking, which is orthogonally applicable to any dialogue model. Specifically, we augment relevant personas to improve dialogue dataset/agent, by leveraging the primal-dual structure of the two tasks, predicting dialogue responses and personas based on each other. Experiments on Persona-Chat show that our approach outperforms pre-trained LMs by an 11.7 point gain in terms of accuracy.

==> table/table1.tex <==
\begin{table*}[t!]
\begin{center}\small
\renewcommand\thetable{2}
{
\begin{tabular}{cccccc}
\hline
  \noalign{\hrule height0.8pt} 
   Dialogue model & Linking model & R@1/20 $\uparrow$ & R@5/20 $\uparrow$ & MRR $\uparrow$ & Contradict@1 $\downarrow$ 
  \TBstrut\\
  \hline
  \noalign{\hrule height0.8pt}
    Bi-encoder & \multirow{2}{*}{N/A} & 0.814 & 0.973 & 0.882 & 0.075  \TBstrut \\
    Cross-encoder &  & 0.884 & 0.991 & 0.930 & 0.040  \TBstrut \\ \hline
    \multirow{4}{*}{Bi-encoder} & Manual Paraphrasing & 0.758 & 0.961 & 0.876 & 0.088  \TBstrut \\
    &Paraphrasing & 0.769 & 0.963 & 0.851 & 0.094  \TBstrut \\
    &Bi-encoder & 0.881 & 0.987 & 0.927 & 0.053  \TBstrut \\
    &Cross-encoder & 0.881 & 0.988 & 0.928 & 0.043  \TBstrut \\ \hline
    \multirow{2}{*}{Bi-encoder} &Persona-Link (small PKB) & 0.904 & 0.992 & 0.943 & 0.039  \TBstrut \\
    &Persona-Link (large PKB) & \textbf{0.931} & \textbf{0.993} & \textbf{0.959} & \textbf{0.027}  \TBstrut \\
  \hline
  \noalign{\hrule height0.8pt} 
\end{tabular}
}
\end{center}
\caption{The performance of dialogue models on Persona-Chat testset}
\label{tab:persona_aug}
\end{table*}


==> table/table2.tex <==
\begin{table*}[t!]
\begin{center}\small
\renewcommand\thetable{2}
{
\begin{tabular}{llccccccccc}
\noalign{\hrule height0.8pt}
  \multicolumn{1}{c}{\multirow{3}{*}{Linking model}} & & \multicolumn{9}{c}{Dialogue model}
    \\   &
  &
  \multicolumn{4}{c}{Pretrained on Wikipedia} &
  \multicolumn{1}{l}{} &
  \multicolumn{4}{c}{Pretrained on Reddit}
  \\ \cline{3-6} \cline{8-11}
\multicolumn{1}{c}{} &
  &
  R@1/20$\uparrow$ &
  R@5/20 $\uparrow$ &
  MRR $\uparrow$ &
  Ctrd.@1 $\downarrow$ &
  &
  R@1/20$\uparrow$ &
  R@5/20 $\uparrow$ &
  MRR $\uparrow$ &
  Ctrd.@1 $\downarrow$ 
  \\
\noalign{\hrule height0.8pt} 
\multicolumn{11}{l}{\textbf{No persona} (0\%)}         \\
N/A        &  & 0.591 & 0.870 & 0.711 & 0.174 &  & 0.659 & 0.900 & 0.766 & 0.144   \\
Bi-encoder &  & 0.699 & 0.936 & 0.802 & 0.120 &  & 0.773 & 0.960 & 0.853 & 0.094   \\
Persona-Link &  & \textbf{0.733} & \textbf{0.956} & \textbf{0.828} & \textbf{0.113} &  & \textbf{0.805} & \textbf{0.970} & \textbf{0.876} & \textbf{0.078}   \\ \hline
\multicolumn{11}{l}{\textbf{Incomplete persona} (80\%)}          \\
N/A        &  & 0.768 & 0.953 & 0.848 & 0.094 &  & 0.825 & 0.973 & 0.889 & 0.073   \\
Bi-encoder &  & 0.768 & 0.966 & 0.850 & 0.094 &  & 0.845 & 0.984 & 0.905 & 0.064   \\
Persona-Link &  & \textbf{0.785} & \textbf{0.972} & \textbf{0.864} & \textbf{0.093} &  & \textbf{0.858} & \textbf{0.985} & \textbf{0.913} & \textbf{0.058}  \\ \hline
\multicolumn{11}{l}{\textbf{Original persona} (100\%)}           \\
N/A        &  & 0.814 & 0.973 & 0.882 & 0.075 &  & 0.868 & 0.986 & 0.919 & 0.054  \\

\noalign{\hrule height0.8pt} 
\end{tabular}
}
\end{center}
% \caption{The performance of a dialogue model on Persona-Chat, where personas are masked out and linking models augment personas only in inference-time.}
\caption{The response quality of Persona-Chat models, observing debiased personas added at test time. In advance, in-dialogue persona sentences were randomly removed, and link models augmented in-context personas based on dialogue histories.}
\label{tab:chat_performance}
\end{table*}

% \begin{table*}[t!]
% \begin{center}\small
% \renewcommand\thetable{2}
% {
% \begin{tabular}{llccccccccc}
% \noalign{\hrule height0.8pt}
%   \multicolumn{1}{c}{\multirow{3}{*}{Rewritten Persona}} & & \multicolumn{9}{c}{Chat Model} \\   &
%   &
%   \multicolumn{4}{c}{Pretrained on Reddit} &
%   \multicolumn{1}{l}{} &
%   \multicolumn{4}{c}{Pretrained on Wikipedia}
%   \\ \cline{3-6} \cline{8-11}
% \multicolumn{1}{c}{} &
%   &
%   R@1/20$\uparrow$ &
%   R@5/20 $\uparrow$ &
%   MRR $\uparrow$ &
%   Ctrd.@1 $\downarrow$ &
%   &
%   R@1/20$\uparrow$ &
%   R@5/20 $\uparrow$ &
%   MRR $\uparrow$ &
%   Ctrd.@1 $\downarrow$ 
%   \\
% \noalign{\hrule height0.8pt} 

% % \multicolumn{11}{l}{\textbf{Original personas} (100\%)}           \\
% % \hline

% % \multicolumn{11}{l}{\textbf{Trained on the original Persona-Chat}} \\

% \hline

% \textit{Full-persona}    &  & 0.868 & 0.986 & 0.919 & 0.054 &  & 0.814 & 0.973 & 0.882 & 0.075  \\ 

% \hline

% % N/A        &  & 0.814 & 0.973 & 0.882 & 0.075 &  & 0.868 & 0.986 & 0.919 & 0.054  \\
% \textit{Few-persona} + Persona-Link &  & \textbf{0.858} & \textbf{0.985} & \textbf{0.913} & \textbf{0.058} &  & \textbf{0.785} & \textbf{0.972} & \textbf{0.864} & \textbf{0.093}  \\
% \textit{Few-persona} + Bi-encoder &  & 0.845 & 0.984 & 0.905 & 0.064 &  & 0.768 & 0.966 & 0.850 & 0.094   \\
% \textit{Few-persona}      &  & 0.825 & 0.973 & 0.889 & 0.073 &  & 0.768 & 0.953 & 0.848 & 0.094   \\

% \hline

% \textit{Zero-persona} + Persona-Link &  & \textbf{0.805} & \textbf{0.970} & \textbf{0.876} & \textbf{0.078} &  & \textbf{0.733} & \textbf{0.956} & \textbf{0.828} & \textbf{0.113}   \\
% \textit{Zero-persona} + Bi-encoder &  & 0.773 & 0.960 & 0.853 & 0.094 &  & 0.699 & 0.936 & 0.802 & 0.120   \\
% \textit{Zero-persona}        &  & 0.659 & 0.900 & 0.766 & 0.144 &  & 0.591 & 0.870 & 0.711 & 0.174   \\

% \hline 


% % \multicolumn{11}{l}{\textbf{Trained on our debiased Persona-Chat}} \\

% % \hline

% % \textit{Few-persona} + Persona-Link &  & \textbf{0.858} & \textbf{0.985} & \textbf{0.913} & \textbf{0.058} &  & \textbf{0.785} & \textbf{0.972} & \textbf{0.864} & \textbf{0.093}  \\
% % \textit{Few-persona} + Bi-encoder &  & 0.845 & 0.984 & 0.905 & 0.064 &  & 0.768 & 0.966 & 0.850 & 0.094   \\
% % \textit{Few-persona}      &  & 0.825 & 0.973 & 0.889 & 0.073 &  & 0.768 & 0.953 & 0.848 & 0.094   \\

% % \hline

% % \textit{Zero-persona} + Persona-Link &  & \textbf{0.805} & \textbf{0.970} & \textbf{0.876} & \textbf{0.078} &  & \textbf{0.733} & \textbf{0.956} & \textbf{0.828} & \textbf{0.113}   \\
% % \textit{Zero-persona} + Bi-encoder &  & 0.773 & 0.960 & 0.853 & 0.094 &  & 0.699 & 0.936 & 0.802 & 0.120   \\
% % \textit{Zero-persona}        &  & 0.659 & 0.900 & 0.766 & 0.144 &  & 0.591 & 0.870 & 0.711 & 0.174   \\

% \hline

% \end{tabular}
% }
% \end{center}
% \caption{The response quality of dialogue models trained on the original Persona-Chat. Before test time, in-dialogue persona sentences were randomly removed and rewritten by linking models based on the utterance history. \textit{Few} means 80\%.}
% \label{tab:chat_performance}
% \end{table*}

==> table/table3.tex <==
\begin{table}[t!]
\begin{center}\small
\renewcommand\thetable{2}
{
\begin{tabular}{l}
\hline
  \noalign{\hrule height0.8pt}
    \textbf{Agent's personas:} \\
    My mom is a secretary. \\
    I am a bodybuilder. \\
    I have one brother. \\
    (-) \sout{I like to eat a lot of meat.} \\
    (+) I am a meat eater. \\
    (+) My favorite meal is steak. \\
    \hline
    \noalign{\hrule height0.4pt}
    \textbf{Dialogue history:} \\
     \emph{User}: Hi there, how are you tonight? \\
     \emph{Agent}: Great. I just finished a huge steak. How are you? \\
     \emph{User}: I am good, drinking some scotch. \\
     \hline
    \textbf{Response without augmented personas:} \\
    \emph{Agent}: Cool! What are your hobbies?\\ %\xmark \\
    \hline
    \textbf{Response with augmented personas:}\\
    \emph{Agent}: I am major meat eater to build muscles.\\ %\cmark \\
  \hline
  \noalign{\hrule height0.8pt}
\end{tabular}
}
\end{center}
\caption{The model calibration in response retrieval task based on online persona augmentation. After removing persona (-), a linking model augmented personas  (+), which calibrates the prediction of dialogue agent, with any parameter updates.}
\label{tab:chat_case}
\end{table}

==> table/table4.tex <==
\begin{table}[t!]
\begin{center}\small
\renewcommand\thetable{2}
{
\begin{tabular}{lcccc }
\hline
  \noalign{\hrule height0.8pt} 
   Linking Model & R@1 & R@10 & MRR 
  \TBstrut\\
  \hline
  \noalign{\hrule height0.8pt}
  Cosine Similarity & 0.108 & 0.349 & 0.190 \TBstrut \\
  BM25 & 0.491  & 0.792 & 0.595 \TBstrut \\
  K-NRM & 0.294  & 0.591 & 0.384  \TBstrut \\
  CONV-KNRM & 0.345  & 0.628 & 0.439 \TBstrut \\
  Bi-encoder & 0.583 & 0.871 & 0.684 \TBstrut \\
  \hline
  Ours (EDA) & 0.599  & 0.885 & 0.709 \TBstrut \\
  Ours (Para) & 0.610  & 0.885 & 0.715 \TBstrut \\
  Ours & \textbf{0.669}  & \textbf{0.922} & \textbf{0.759} \TBstrut \\
  \hline
  \noalign{\hrule height0.8pt} 
\end{tabular}}
\end{center}
\caption{Linking performance on Persona-Link}
\label{tab:performance}
\end{table}


==> table/table4_backup.tex <==
\begin{table}[t!]
\begin{center}\small
\renewcommand\thetable{2}
{
\begin{tabular}{lcccc }
\hline
  \noalign{\hrule height0.8pt} 
   Linking Model & R@1 & R@10 & MRR & Avg 
  \TBstrut\\
  \hline
  \noalign{\hrule height0.8pt}
  Cosine Similarity & 0.108 & 0.349 & 0.190 & 0.270 \TBstrut \\
  BM25 & 0.491  & 0.792 & 0.595 & 0.694 \TBstrut \\
  K-NRM & 0.294  & 0.591 & 0.384 & 0.487  \TBstrut \\
  CONV-KNRM & 0.345  & 0.628 & 0.439 & 0.533 \TBstrut \\
  Bi-encoder & 0.583 & 0.871 & 0.684 & 0.777 \TBstrut \\
  \hline
  Ours (EDA) & 0.599  & 0.885 & 0.709 & 0.797 \TBstrut \\
  Ours (Para) & 0.610  & 0.885 & 0.715 & 0.800 \TBstrut \\
  Ours & \textbf{0.669}  & \textbf{0.922} & \textbf{0.759} & \textbf{0.840} \TBstrut \\
  \hline
  \noalign{\hrule height0.8pt} 
\end{tabular}}
\end{center}
\caption{Linking performance on Persona-Link}
\label{tab:performance}
\end{table}

